Learning From Software Failures: A Case Study at a National Space Research Center

Software failures can have significant consequences, making learning from failures a critical aspect of software engineering. While software organizations are recommended to conduct postmortems, the effectiveness and adoption of these practices vary widely. Understanding how engineers gather, document, share, and apply lessons from failures is essential for improving reliability and preventing recurrence. High-reliability organizations (HROs) often develop software systems where failures carry catastrophic risks, requiring continuous learning to ensure reliability. These organizations provide a valuable setting to examine practices and challenges for learning from software failures. Such insight could help develop processes and tools to improve reliability and prevent recurrence. However, we lack in-depth industry perspectives on the practices and challenges of learning from failures. To address this gap, we conducted a case study through 10 in-depth interviews with research software engineers at a national space research center. We examine how they learn from failures: how they gather, document, share, and apply lessons. To assess transferability, we include data from 5 additional interviews at other HROs. Our findings provide insight into how engineers learn from failures in practice. To summarize: (1) failure learning is informal, ad hoc, and inconsistently integrated into SDLC; (2) recurring failures persist due to absence of structured processes; and (3) key challenges, including time constraints, knowledge loss from turnover and fragmented documentation, and weak process enforcement, undermine systematic learning. Our findings deepen understanding of how software engineers learn from failures and offer guidance for improving failure management practices.

==> data/raw_results.tex <==
\myparagraph{Failure knowledge discussion practices are ad hoc}
\iffalse
Most case study participants (9/10) reported that failure discussions lack structure and occur informally. 
Half of them (5/10) provided specific examples of these ad hoc discussions, highlighting their inconsistent nature across teams and projects.
A senior team member, Subject 1, shared that their original plan for structured failure meetings never materialized due to overwhelming technical debt:
"I originally thought when we set up those meetings...we will go through all issues in discussion and then they will be either closed or open and then we can work on them...But this never happened because the technical debt was too large too much for us and it took us too much time to discuss."
Subject 3 described how failure discussions occur during "team meetings" only when, "the developer brings it up if they want to" and vary by project size -- "this kind of communication, but it's not in every project, but in some projects" -- and available resources -- "depends actually how big the project is, right?...So sometimes we have very small budgets...So there you don't need a process, you just call them...then let's say larger development things, you probably need some more formalized stuff."
The depth of these discussions also depends on leadership influence, as noted by Subject 2:
"coming from the influence of group leader and department...to bring this practice to your group that they don't hesitate to report problem and discuss it and come up with the lesson learned and that's because it will help your group to grow. That's actually nothing standard, nothing written."
While there is an effort to improve failure discussions, structure remains uncertain. 
For instance, Subject 8 mentioned an upcoming organization-wide meeting on software practices but was unsure about its format:
"I think I'm expecting, actually not sure because I'm not planning there agenda of this meeting, but we are going to discuss about the process. At least I have some feedback from that, how we can improve what are maybe kind of our bottlenecks during development and also maybe how to discuss the implementation of some blocks."
Some participants reported that discussions on lessons learned rarely happen at all. 
When asked about when such discussions occur, Subject 6 stated:
"Yeah, this will mostly, yeah, this rarely will occur. I have never been in a situation like that," and that "we don't have a very strict process for that, to be honest. Not really."
\fi

\myparagraph{Failure knowledge documentation practices are ad hoc}




\iffalse
Most case study participants (8/10) reported that failure documentation practices are not standardized and are ad hoc. 
Several participants reported that there is no formalized process for documenting failure knowledge and lessons learned, and is often left to individual discretion. 
Subject 4 explained that documentation is not mandatory and remains a personal choice:
"And when we close the issue, it is not mandatory to document what did you do or create these kind of examples. I think that's something more personal decisions...We don't have that process integrated in our system. So me personally, I know from experience that this is really important so I do it."
This sentiment was echoed by Subject 11, who emphasized the need for standardization:
"I think firstly maybe you have to standardize what you should write."
When asked about documentation practices for lessons learned, Subject 6 admitted that they rarely occur:
"Oh, I don't think they are documented, pretty much at all. No, I think that there should be more a formal process at least on how to do that."
Even when documentation does exist, there is no defined process for ensuring consistency, as Subject 3 noted:
"Yes, it might be, but it's not like there's a process for that."

Half of the participants (5/10) described various methods used to capture failure knowledge, highlighting that such knowledge is distributed across multiple platforms and lacks standardization.
According to all participants, GitLab is the primary tool for storing failure knowledge. 
However, other tools and locations are also used, leading to fragmented documentation. 
The most senior participant (S7) shared that failure insights are sometimes recorded in formal scientific documents:
"Sometimes...I'm writing down in some scientific documents...[and] publications showing the lessons learned... [and] white papers on ideas what's going wrong and what could be better."
Another participant (S4) echoed this sentiment, emphasizing the benefits of the publication process in uncovering issues:
"Thanks to the publication process...we discovered some issues."
Several participants highlighted that merge requests also contain failure-related discussions, as Subject 4 noted:
"There are also discussions in the merge request."
Wikis were mentioned as another documentation method, though their use varied across teams. 
Subject 2 described how some teams create wiki pages and attach meeting slides:
"Maybe in a sort of minutes of the meeting because usually we create a wiki page for such a meeting and we take notes...Usually the people reporting may have a few slides also they attach to this wiki page."
However, not all projects have a dedicated failure knowledge wiki, making this approach inconsistent:
"Really, when you look to the wiki page called ‘lesson learned from project,’ it's a few, not every project has one, but that’s the way of taking notes on a wiki page."


Beyond the lack of standardization, participants also expressed confusion over where failure knowledge is stored, making it difficult to retrieve and reference past failure knowledge and lessons.
Subject 5 expressed uncertainty about where different types of failure-related information are stored:
"I knew that there is a GitLab, but I didn't know what was documented in GitLab, what was documented in the wiki, what was documented on the team side, and what was discussed in which meeting."
Subject 5 further explained that where an issue is recorded depends on its scale and significance:
"So if it's one of those bigger issues with the architecture, then it might get its own GitLab issue. Or if it's big enough to be discussed in the meeting with the other institutes, then it gets in the meeting notes. If it's just a local discussion focused on a single application or something, then I don't think it gets documented."
Some participants confirmed that issues and lessons learned are not systematically stored. 
When asked about storage practices, Subject 2 stated:
"Again, they're not really stored, they're just presented.
When documentation does exist, it is often in informal formats, such as meeting notes or wikis, as Subject 2 explained:
"At best, they are just on a wiki page."
The most senior participant (S7) mentioned contributing failure knowledge to a software engineering network within the organization, but this resource was not referenced by any other participants, suggesting low awareness or usage:
"Today I would use wiki. Yeah. And I also share my experiences inside wiki. We have the software engineering network and several lessons learned inside the software engineering network coming from me with my experiences also."
\fi

\iffalse
Most case study participants (8/10) reported that failure documentation practices are not standardized and are ad hoc. 
Half of them (5/10) share various methods that are used to capture failure knowledge, showing that such knowledge is distributed and not standardized.  
According to all subjects, Gitlab is used to store most failure knowledge, however other tools and places are also used to store failure knowledge. 
For example, the senior most subject (S7) shares that they "Sometimes...I'm writing down in some scientific documents...[and] publications showing the lessons learned... [and] white papers on ideas what's going wrong and what could be better," and the benfits of this sentiment is shared by another subject (S4), "thanks to the publication process...we discovered some issues."
Some participants reported that documentation of lessons learned rarely happens at all. 
When asked about when such documentations occur, (S6) stated:
"Oh, I don't think they are documented, pretty much at all. No, I think that there should be more a formal process at least on how to do that."
Confirmed by S11:
"I think firstly maybe you have to standardize what you should write"
Confirmed by S4:
"And when we close the issue, it is not mandatory to document what did you do or create these kind of examples. I think that's something more personal decisions...We don't have that process integrated in our system. So me personally, I know from experience that this is really important so I do it"
SOme subjects (S4) also highlight the failure knowledge that is documented in: "there are also discussions in the merge request." 
When asked if the solution to an issue is documented, a subject (S3) responds,"yes, it might be, but it's not like there's a process for that."
Subject 5 says, "I knew that there is a GitLab, but I didn't know what was documented in GitLab, what was documented in the wiki and what was documented on the team side and what was discussed in which meeting."
Subject 5 also says, "So if it's one of those bigger issues with the architecture, then it might get its own GitLab issue. Or if it's a big enough to be discussed in the meeting with the other institutes, then it gets in the meeting notes. If it's just a local discussion focused on a single application or something, then I don't think it gets documented."
When asked about how issues and lessons learned are stored subject 2 says, "Again, they're not really stored, they're just presented." but then says, "at best, they are just on a wiki page."
Subject 2 also says, "Not always. Maybe in a sort of minutes of the meeting because usually we create a wiki page for such a meeting and we take minutes notes, maybe not really minutes, but notes on that. Usually the people reporting may have few slides also they attach it to this wiki page. Few of them of course. Really when you look to wiki the page called lesson learned from project, it's a few, not every project has one, but that's the way of the taking notes on a wiki page."
The most senior member, subject 7 also says, "Today I would use wiki. Yeah. And I also share my experiences inside wiki. We have the software engineering network and several lessons learned in inside the software engineer network coming from me with my experiences also," however none of the other subjects refered to this knowledge.
\fi

\iffalse
Most of the case study subjects (9/10) share that the discussions they have for failures are ad hoc in structure. 
And half of the case study subjects (5/10) shared specific examples of ad hoc failure discussions.
For example, a senior member (S1) of the team reports that the original structure they had planned for their failure discussion meetings veered off in practice, "I originally thought when we set up those meetings...we will go through all issues in discussion and then they will be either closed or open and then we can work on them...But this never happened because the technical debt was too large too much for us and it took us too much time to discuss."
Another member (S3) shares that discussions about issues happen during "team meetings, the developer brings it up if they want to" and these discussions varies from one project to another, "this kind of communication, but it's not in every project, but in some projects" and that such discussions happen based on resources available "depends actually how big the project is, right?...So sometimes we have very small budgets...So there you don't need a process, you just call them...then let's say larger development things, you probably need some more formalized stuff."
Another subject (S2) shares that such discussions are structured to different degrees of depth, "coming from the influence of group leader and department...to bring this practice to your group that they don't hesitate to report problem and discuss it and come up with the lesson learned and that's because it will help your group to grow. That's actually nothing standard, nothing written."
Another subject (S8) mentions the first ever upcoming organization wide meeting about software practices  to discuss failures, lessons learned etc., but is unsure about how it will be structured or what will actually be discussed, "I think I'm expecting, actually not sure because I'm not planning there agenda of this meeting, but we are going to discuss about the process. At least I have some feedback from that, how we can improve what are maybe kind of our bottlenecks during development and also maybe how to discuss the implementation of some blocks. Yeah."
When asked about when the discussion of lessons learned happens, another subjects (S6) says, "Yeah, this will mostly, yeah, this rarely will occur. I have never been in a situation like that," and that "we don't have a very strict process for that, to be honest. Not really."
\fi


\subsection{Theme 2: Failure knowledge transfer practices are unstructured} 
All case study participants reported that failure knowledge transfer practices are unstructured and occur on an ad hoc basis.
Within teams, engineers primarily share knowledge through informal conversations rather than structured processes. 
Subject 4 described how failure knowledge is shared through casual interactions rather than formal reporting, "I will say that not officially, but it is common that during the day I discuss something with my team members, like my office mate or something like that, but not in an official way."
Subject 9 corroborates, "Yeah, yeah, it's more like just Okay, just on the go."
Subject 5 reinforced the ad hoc nature of internal knowledge sharing, explaining that engineers typically communicate issues only when they need assistance, "So if you have an issue, you basically tell the other people in your team that you have an issue, what exactly the problem is. Depending on if you expect them to help you or not, you can go into detail or not. And if they have an idea or if they encountered that issue before, then they will tell you. And maybe you make, if you have one person who says, 'Okay, I know how to deal with it,' then you can make a follow-up meeting with just that person. So you don't need to discuss it with everybody. I think that's more or less how it goes most of the time."
A few participants reported that stand-up meetings provide a space to share obstacles and failure knowledge, but this is inconsistent across projects. 
Subject 3 described the variability in this practice, "Stand-up meetings where...discussing...obstacles...the discussion is to know also, okay, what if someone has had the problem before or if someone has an idea how to solve the problem. So this kind of communication, but it's not in every project."

Failure knowledge is rarely shared beyond the immediate team, and there is little formalized communication between teams or organizations. Subject 1 noted that failure reports in broader project meetings are uncommon and often met with disinterest, "Very rarely we report in a bigger round for the project that we experienced a failure or a problem and that we fixed it...the interest in that is also very low...So it completely stays in the team and will not be exchanged with others."
When asked whether failure knowledge is shared to prevent mistakes from recurring in other projects, Subject 2 emphasized that it depends on the severity and relevance of the issue, "I mean mainly depending on the criticality and relevance, I say it is clearly, if it's relevant for other projects or a very critical situation, then this information is spread in the group...we are trying to overcome it this way."
Subject 5 echoed this sentiment, explaining that engineers avoid sharing minor issues externally to avoid unnecessary meetings, "You don't want to bore all the 20 people from other institutes with something that is probably not relevant for them."
Subject 3 explained how knowledge transfer occurs across projects, "Within the project...Well, it depends very much on the project, how it's organized...let's say I work in one project, get some experience with certain part of problems, start working on another project, and of course I bring this experience with it and try to communicate this."
Some participants mentioned that failure knowledge is occasionally shared in Brown Bag Lunch (BBL) meetings, though these are sporadic rather than regular practice. Subject 2 stated, "BBL [Brown Bag Lunches - lunch and learn] meeting actually this sporadic one, not regular one."

All participants mentioned that the primary method of failure knowledge transfer is through senior engineers mentoring junior members. 
The most senior team member, Subject 7, was frequently cited as the go-to person for resolving issues. 
A junior engineer, Subject 9, described their reliance on Subject 7, "In the beginning, till I get a better feeling for it, I would always check with [Subject 7], 'Hey, how would you do it? Do you have any experience? What's the common way? What's best practice?' Yeah, that's the approach."
When asked how past failures are avoided, Subject 9 added, "Yeah, but I also have to ask [Subject 7] for examples" and "he sharing his experience and we can then decide how we want to avoid problems or how we want to improve something."
Subject 6 described how knowledge transfer is largely dependent on direct interactions rather than documentation, "Basically the way is...I have this issue...I could just go to [Subject 7's] office and ask, okay, we have this issue, how would you tackle it? What do you think?...But yeah, normally it's just knocking at the door and asking, 'Hey, do you have any experience on these type of things?'"
Subject 5 stated that this informal system works well for now, "A lot of it is communication because we have some really experienced developers in the team. So when I have an issue, I usually...try to ask the people that are more experienced, and until now, that worked pretty well."
Subject 3 talks about the importance of this, "Yeah, there should be [direct knowledge transfer], I mean that's how you grow as a developer, right? By getting maybe some influence by some similar experience."
While senior engineers play a critical role in knowledge transfer, Subject 1 noted that this approach can lead to inefficiencies in resolving recurring failures, "A couple of situations which we had in the last couple of years where issues in our software popped up and sometimes they were recurring...So we experienced that someone was working on the software and he didn't fix it and he asked someone else on the team. And this one then said basically, 'Oh yeah, I remember that I faced this too. You have to do this and that.' So that's probably the worst case, how to handle those things, but that's how it was done actually."
They also highlighted the difficulty of obtaining insights from past failures with such practices, "It's like you have to hope and demand for this knowledge, so you have to ask other people if they experienced that and you got to hope that someone already experienced it or not."
They say, "This could happen only if the person who either fixed it or who was there in the discussion with members. I never experienced that, to be honest, that someone says like, oh yeah, we had this issue before and we fixed it like this and this and we can do it, but there's not a process to look it up to."
Subject 8 shares a similar drawback, "its on the fly...if we or anyone sees something, it is shared, maybe you can do this in this way and you can avoid this," and otherwise its not.

Although subjects admit the importance of ad hoc transfer of failure knowledge from experienced members, since (Subject 2:) "they have all the lessons learned in [their] mind," subjects noted that sharing of failure knowledge should be formally integrated into training to ensure that lessons learned are retained and systematically transferred.
The most experienced member, Subject 7, emphasized the importance of mentoring junior engineers and passing down lessons learned, "This is then more than a training issue. I think experience from the old colleagues must be also taught to the new ones, and it's also one of the reasons why [Team Lead] put me most of the time also in new projects and so on, so that I can share my experience."
They also actively encourage junior engineers to reflect on lessons learned, "Working together then with colleagues and also, yeah. Okay. Then teaching them and so on...I also request them, 'Okay, what do you think? What was going good? What was going bad?' and so on."
Subject 4 described their approach to documenting lessons learned for training purposes, 
"as a more senior member and mentoring younger members...I realized I have to explain again and again and again why I did that. So it's better to document that. And I noticed that the, they were doing something similar [mistakes as] when I started..., so I like to document the important fixes with examples and some documents that explain how the examples were and why the examples were in that way. I use that for training."
However, this is not common practice and is often varied in practice. 
Subject 2 says but is not done often, "We save the problem...[and] sometimes lesson learned before and those are referred when someone new join...but again, that means it's not too often...The last time we referred to some reason was already two years ago or something."
Subject 1 says that "we don't have a lessons learned page or database or something like that, which we guide them to."
Subject 9, one of the newest members, corroborates this saying, "No, as a newcomer for me, I wouldn't know. So it's not written anywhere, it's just the experience from the senior developers." when asked if past documentation or advice is provided about past issues to learn from, and confirmed by Subject 11 another new member, "probably not as actively aware of."


\iffalse

%%%%%%%%%%%%%%%%%%%
All case study participants share that failure knowledge transfer practices are unstructured and are ad hoc. 
When asked if issues are communicated to other teammates, Subject 4 says, "I will say that not officially, but it is common that during the day I discuss something with my team members, like my office mate or something like that, but not in an official way."

When asked how common pitfalls and lessons learned are shared, Subject 8 says, "On the fly..Yeah, if we see something or if anyone sees something, it is shared, maybe you can do this in this way and you can avoid this or it's better somehow."

When asked if issues that are communicated to other teams or other stakeholders do prevent that sort of issue from happening to other people, Subject 3 says, "Within the project...Well, it depends very much on the project, how it's organized. If it's a very open collaboration or a bit more, everyone does their own thing and then someone has the great privilege to try to put everything together. Then after everyone worked for two years on their own or otherwise, it's more like if, let's say I work in one project, get some experience with certain part of problems, start working on another project, and of course I bring this experience with it and try to communicate this."

When asked if failure knowledge is shared outside of the team, Subject 1 says, "Very rarely we report in a bigger round for the project that we experienced a failure or a problem and that we fixed it. But usually the interest in that is also very low in this round, so nobody's really interested in the details there. So it completely stays in the team and will not be exchanged with others"

Subject 1 also says that if you need experienced insight on a problem, "it's like you have to hope and demand for this knowledge, so you have to ask other people if they experienced that and you got to hope that someone already experienced it or not."


All subjects state the primary form of failure knowledge transfer is though senior members internalizing failure knowledge and then transferring it to junior members. 
All subjects mentioned going to Subject 7, the most senior member on the team for such ad hoc knowledge transfer, 
One of the junior most members, Subject 9, shares that, when faced with issues or for good practice "in the beginning till I get a better feeling for it, I would always check with [Subject 7] Hey, how would you do it? Do you have any experience? What's the common way? What's best practice? Yeah, that's the approach."
And when asked if they try to prevent issues from the past and how they do it, "Yeah, but I also have to ask you to ask [Subject 7] for examples" and "he sharing his experience and we can then decide how we want to avoid problems or how we want to improve something."

Subject 1 shares that such unstructured knowledge transfer process leads to inefficient resolution process when faced with recurring issues: "a couple of situations which we had in the last couple of years where issues in our software popped up and sometimes they were recurring...So we experienced that someone was working on the software and he didn't fix it and he asked someone else on the team. And this one then said basically, oh yeah, I remember that I faced this too. You have to do this and that. So that's probably the worst case, how to handle those things, but that's how it was done actually."

Subject 5 says that, "So if you have an issue, you basically tell the other people in your team that you have an issue what exactly the problem is, depending on if you expect them to help you or not, you can go into detail or not. And if they have an idea or if they encountered that issue before, then they will tell you. And maybe you make, if you have one person who says, okay, I know how to deal with it, then you can make a follow-up meeting with just that person. So you don't need to discuss it with everybody. I think that's more or less how it goes most of the time."

And when asked if they share failure knowledge so mistakes arent repeated, Subject 2 says, "I mean mainly depending on the criticality and relevant I say it is clearly there's relevant for other projects or very critical situation. Then this information on spreading the group, that's actually it was critical and we are trying to overcome it this way." Subject 5 shares the similar sentiment that "You don't want to bore all the 20 people from other institutes with something that is probably not relevant for them."

Subject 3 shares how ad hoc the problem helping knowledge transfer is across different projects:
"stand up meetings where...discussing...obstacles...the discussion is to know also, okay, what if someone has had the problem before or if someone has an idea how to solve the problem. So this kind of communication, but it's not in every project"

When asked if there was a process for getting past failure knowledge or design insight from an experiences member, Subject 9 says, "Yeah, yeah, it's more like just Okay, just on the go."


Subject 4 says that they use past failure knowledge for training new members, and they "like to document the important fixes with examples and some documents that explain how the example were and why the example were in that way. I use that for training." and " And then I started to work with, I don't know, as a more senior member and mentoring younger members. And then I realized, ah, okay, I have to explain again and again and again why I did that. So it's better to document that. And I noticed that the, they were doing something similar when I started...for example, there were a set of examples"
And this is also something Subject 2 says but is not done often, "We save the problem...[and] sometimes lesson learned before and those are referred when someone new join...but again, that means it's not too often...The last time we referred to some reason was already two years ago or something."

Subject 1 contradicts this by saying, "we don't have a lessons learned page or database or something like that, which we guide them to."
Which Subject 9, one of the newest members, agrees to, "No, as a newcomer for me, I wouldn't know. So it's not written anywhere, it's just the experience from the senior developers." when asked if past documentation or advice is provided about past issues to learn from, and confirmed by Subject 11 another new member, "probably not as actively aware of."

Subject 3 talks about the importance of this, "Yeah, there should be [direct knowledge transfer], I mean that's how you grow as a developer, right? By getting maybe some influence by some similar experience"

Subject 1, one of the senior engineers, contradicts the rest of the knowledge transfer practices shared by saying, "Only if the person who either fixed it or who was there in the discussion with members only then this could happen. I never experienced that, to be honest, that someone says like, oh yeah, we had this issue before and we fixed it like this and this and we can do it, but there's not a process to look it up to say, okay, let's just ask a database might be that this was already fixed." But they recount a time where they were able to help with an issue based on past experience, "It was more like someone called me and asked, here I have this and that issue. Have you ever experienced that? And I basically helped them, but further than that, we didn't take any measures to prevent that" - Showing that this may not really be a general practice.

The most experienced member Subject 7 shares that, "This is then more than a training issue. I think experience from the old colleagues must be also taught to the new ones and it's also one of the reasons why [Team Lead] put me most of the time also new projects and so on so that I can share my experience."
And they share that they try to do this, "Working together then with colleagues and also, yeah. Okay. Then teaching them and so on...I also request them, okay, what do you think? What was going good? What was going bad and so on."


Subject 6 shares that, "basically the way is...I have this issue...I could just go to [Subject 7's] office office and ask, okay, we have this issue, how would you tangle it? What do you think?...But yeah, normally it's just knocking at the door and asking, Hey, do you have any experience on these type of things." and shares an example instance, "by senior members on the team like [team member] or [team member] for example, who is also sometimes helping us and there are constant reference by them, oh [in past project] this was done this way maybe should done this way. And I see there is always reference to these things." rather than looking at past failure knowledge documentation.

Subject 5 says that such ad hoc failure knowledge sharing has been working pretty well, "A lot of it is communication because we have some really experienced developers in the team. So when I have an issue, I usually...try to ask the people that are more experienced and until now, that worked pretty well."

Subject 2 emphasizes the importance of "what helps so far same seniors are still in the group. They have all the lessons learned in mind."

A few subjects also mention that failure knowledge and lessons learned are also shared ad hoc during (Subject 2:) "BBL [Brown Bag Lunches - lunch and learn] meeting actually this sporadic one, not regular one." 
\fi




\iffalse
\SubjectFive says that, \myinlinequote{I don't think that we have a formal process on how to make sure that it doesn't happen again.}
When asked about if there are any efforts to learn from failures, they say, \myinlinequote{Not as far as I know...I mean, we have processes for everything and I guess it would be helpful to have a process to learn from mistakes regarding code quality because it probably takes a lot of time if people make the same mistakes over and over again} and adds that it would be nice to incorporate within training, 
\myinlinequote{I feel like a process somewhere embedded in the on-boarding process of new employees would definitely help.}
%\myinlinequote{It's not like it's in the on-boarding process or something, but I think that would be really, really helpful to have.}
However, they add that, \myinlinequote{I gave...feedback...so now there are some improvements being made...But I guess those not those steps that are being taken are not in a process defined by itself, but they are more on the personal motivation of some developers}, showing that continuous improvements are made as a result of personal lessons learned and application rather than as a part of continuous improvement development processes.


When asked when they if they discuss preventing severe issues and if they discuss what the lessons learned are, \SubjectSix says, \myinlinequote{this rarely will occur. I have never been in a situation like that. I guess this will happen...we don't have a very strict process for that, to be honest. Not really}

\SubjectNine is also unsure of whether such a process exists, "But I actually don't, I know it happens, but actually I think [\SubjectSeven] can tell more about this. Yeah, if you want to have any examples, maybe ask him for this. He has to better overview."

\DA{Repeated quote here - but it fits better here}
\SubjectOne shares that there is a need for a process to learn from failures to prevent recurring failures and how the current ad hoc way is inefficient, \myinlinequote{there were a couple of situations which we had in the last couple of years where issues in our software popped up and sometimes they were recurring, so sometimes I saw them again and again, but there wasn't actually a process how to handle those. So we experienced that someone was working on the software and he didn't fix it and he asked someone else on the team. And this one then said basically, oh yeah, I remember that I faced this too. You have to do this and that. So that's probably the worst case, how to handle those things, but that's how it was done actually.}

\SubjectThree says, \myinlinequote{It's not that much that there's a big reflective period where we say, okay, this error happened and now how should we do that now in the future...it's not, so the reflection part that you come together as a group and let's say now reflect on the bug you notice or something is usually not part of the things}

When asked if they gather lessons learned for continuous improvement, \SubjectEight says, \myinlinequote{No, I can recall. I mean, we're going to do this actually in a couple of weeks. We have a business trip and we're going to, and in this partner projects, we work with milestones and we are going to meet and discuss what are the results of the first milestone, give some feedback and try to see how we continue with the next. So I think I don't have a recall, but in two weeks I will have one...[But] No? No, it is not standard. Yeah, it's not standard, but I think it's a good way to see how we can improve...No, it's software specific. Yes...I think I'm expecting, actually not sure because I'm not planning there agenda of this meeting, but we are going to discuss about the process. At least I have some feedback from that, how we can improve what are maybe kind of our bottlenecks during development and also maybe how to discuss the implementation of some blocks. Yeah...} and that this is the first time they've been a part of something like this at DLR.
But in general, they say that they don't have such discussions or processes, \myinlinequote{No, I guess no, we don't have that. Got it. Speaker 4 (11:03): Sure. Speaker 2 (11:04): No, I'm thinking that maybe there is something I don't know important to share. We have this space, this slot, I think during Mondays it's called a BBL for discussing or presenting something interesting. So that will be the space. But lately, yeah, we don't use that for this}
When asked if other teams do this, the subject adds, \myinlinequote{Actually, I don't know. Okay. I don't know. Yeah, I think some kind of feedback is needed, but I think every group is dealing with this in their way. It's like we don't have a process.}

When asked about reflective processes to learn from failures, \SubjectFour says, \myinlinequote{Yeah, good point. We are not doing that I think,} which they attribute to, \myinlinequote{Yeah, because we are not following this totally agile approach...that process, no, we don't do that. Got it...usually in this kind of space project you don't see total agile. It's not the case.}
They add, \myinlinequote{I would like to, but I think at least my project is not the case. Got it. Okay. Yeah, I like the idea, but we don't do that.}
\fi


\iffalse
\subsubsection{Theme 3.3: Lessons are documented poorly}

\SubjectEight described that lessons learned are often implicit rather than formally documented:
\myinlinequote{I mean just from implicit, not explicit, but implicit. Okay. I know that some kind of pattern or doing the thing in some way could be dangerous and you learn how to do it in a better way, but this is just internally knowledge your learning. But yeah, I'm not like if I, for example, document how I implemented the issue...[or lessons] No.}

When discussing using common issues and lessons learned, \SubjectEight says, "I mean just from implicit, not explicit, but implicit. Okay. I know that some kind of pattern or doing the thing in some way could be dangerous and you learn how to do it in a better way, but this is just internally knowledge your learning. But yeah, I'm not like if I, for example, document how I implemented the issue...[or lessons] No."

When asked if there's lesson learned documentation, \SubjectFive responds, "Not in the project that I've worked with so far," \SubjectTwo responds, "We track issues, but yeah, not for lesson," \SubjectTen says, "no really lessons learned, no. I think they're more like internally...we learned from it.

\SubjectTen describes a discussing about a recurring problem, and when asked if the lessons learned was documented, they respond, "it was more just a discussion I would say. I think there wasn't an active writing down, let's not do this again."

\SubjectSix describes a recurring problem and when asked if the lessons learned for it was documented, they say, "I don't think we document it anywhere to be honest. No, I don't think so. Maybe it would be a good idea."

\SubjectOne says, "we don't have a lessons learned page or database or something like that."

When asked if lessons learned are documented, \SubjectTwo responds "No. No. Do not see lesson learned. You'll find the discussions [in issue reports,] but not explicitly referred that this is lesson learned from this project."

\SubjectSix recounts a general (not just software) post-mission debrief meeting, and when asked if lessons learned from this meeting are documented, \SubjectSix says, "So this general meeting was documented with general minutes of meeting," and when asked about documentation practices for lessons learned, \SubjectSix admitted that they rarely occur:
\myinlinequote{Oh, I don't think they are documented, pretty much at all. No, I think that there should be more a formal process at least on how to do that.}

\DA{Quotes about documentation for lessons learned should be moved here from 5.1 I think }

\DA{Quote is repeated, but there's another quote that could be switched in: "So that I have also there are some publications that showing the lessons learned"}
When asked if they document the lessons they gather implicitly, the senior most \SubjectSeven says, "Sometimes yes and some scientific documents that I'm writing down...is lessons learned from the previous project...and writing also white papers...on the ideas what's going wrong and what could be better"
"Today I would use wiki...[to] share my experiences inside wiki. We have the software engineering network and several lessons learned in inside the software engineer network coming from me" However, the other subjects rarely mentioned such lessons learned wiki.

\SubjectNine says, "I know we document lessons learned in the project phases. I think it's happening at the end of every milestone or so. So I had this for other projects regarding the requirements, but we concluded we derived lessons learned from it and put in another document...it's more like the whole project than for the software development. I'm not sure if something like this exists." when probed further on what such documentation consists, the subject says, "just a general description of the issue and what the suggestions were. But overall pretty general," which is not really lessons learned. 

When asked whether the lessons learned from the organization-wide meeting on software practices will be documented, \SubjectEight responds, "No, I think...probably we'll take notes. Not sure if there will be a minutes taker or something. I don't think so really, but probably, I mean everyone is taking notes."

\SubjectOne asks, "how to document learnings, that is probably something also, this is a hurdle. How do we document that?"

When asked how the lessons learnt are stored, \SubjectTwo says, "they're not really stored, they're just presented...best way, they are just on a wiki page."

When asked about the most problematic part of the learning from failures process, \SubjectTwo responds, \myinlinequote{As we maybe conclude, we can conclude from all this discussion. Actually this knowledge could be lost because they are not well documented and not well not processed to transfer it in a process. Right. And sometimes it's, yeah, it's ongoing on go some project they are okay, we are just tired. Maybe we do it next month after we finish the project, we got three weeks to go to Canary Islands. Then maybe we'll do it in the after pack. They are cutting new project and forget that one and then actually it's gone because there's no process to say no, part of your project is to write lesson learned.}

\DA{Repeated but better fit here}
When asked how lesson learned are documented, \SubjectTwo says, "Not always. Maybe in a sort of minutes of the meeting because usually we create a wiki page for such a meeting and we take minutes notes, maybe not really minutes, but notes on that. Usually the people reporting may have few slides also they attach it to this wiki page. Few of them of course. Really when you look to wiki the page called lesson learned from the project, it's a few, not every project has one, but that's the way of the taking notes on a wiki page. As a minutes of the meeting discuss the points discussed in the meeting, the main points of the meeting, like the problem, the conclusion and sometimes I said we will have at least I have in mind one example that's actually well search problem and solution and lesson learned documentation, but that's actually not standard, not always."

\fi

==> data/results_extended.tex <==
\section{Results and Analysis} \label{sec:Results}
We organize our results into themes that answer our research questions. 
\DA{I think we may have to define failure knowledge?}

\subsection{Theme 1: Failure knowledge discussion and documentation practices are unstructured} 
\JD{Perhaps just ``Characterization of process''. Jamie will take a pass here.}
%In this section, we aimed to understand how practitioners discuss and document their failure knowledge.

\DA{Most subject also talk about open failure culture - we have a code for it if we want to talk about it. 
An example of how failure discussions start:
"And then basically we initiate a conversation normally in the form of an email or we organize kind of meeting and to try to figure out where the issue comes from and who's responsible for it and who will investigate. Most of the time they send in kind of a playing game to pass a blame to everybody. But yeah, sometimes we're civilized" - But the rest of subjects say that there's open failure culture.
}

%\myparagraph{Failure knowledge discussion practices are ad hoc}
Most case study participants (9/10) reported that \ul{failure discussions lack structure and occur informally.} 
Half of them (5/10) provided specific examples of these ad hoc discussions, highlighting their inconsistent nature across teams and projects.
A senior team member, \SubjectOne, shared that their original plan for structured failure meetings never materialized due to overwhelming technical debt:
\myinlinequote{I originally thought when we set up those meetings...we will go through all issues in discussion and then they will be either closed or open and then we can work on them...But this never happened because the technical debt was too large too much for us and it took us too much time to discuss.}
\SubjectThree described how failure discussions occur during \myinlinequote{team meetings} only when, \myinlinequote{the developer brings it up if they want to} and vary by project size -- \myinlinequote{this kind of communication, but it's not in every project, but in some projects} -- and available resources -- \myinlinequote{depends actually how big the project is, right?...So sometimes we have very small budgets...So there you don't need a process, you just call them...then let's say larger development things, you probably need some more formalized stuff.}
The depth of these discussions also depends on leadership influence, as noted by \SubjectTwo:
\myinlinequote{coming from the influence of group leader and department...to bring this practice to your group that they don't hesitate to report problem and discuss it and come up with the lesson learned and that's because it will help your group to grow. That's actually nothing standard, nothing written.}
While there is an effort to improve failure discussions, structure remains uncertain. 
For instance, \SubjectEight  mentioned an upcoming organization-wide meeting on software practices but was unsure about its format:
\myinlinequote{I think I'm expecting, actually not sure because I'm not planning there agenda of this meeting, but we are going to discuss about the process. At least I have some feedback from that, how we can improve what are maybe kind of our bottlenecks during development and also maybe how to discuss the implementation of some blocks.}
Some participants reported that discussions on lessons learned rarely happen at all. 
When asked about when such discussions occur, \SubjectSix stated:
\myinlinequote{Yeah, this will mostly, yeah, this rarely will occur. I have never been in a situation like that,} and that \myinlinequote{we don't have a very strict process for that, to be honest. Not really.}



%\myparagraph{Failure knowledge documentation practices are ad hoc}
Most case study participants (8/10) reported that \ul{failure documentation practices are not standardized and are ad hoc.}
Several participants reported that there is no formalized process for documenting failure knowledge and lessons learned, and it is often left to individual discretion. 
\SubjectFour explained that documentation is not mandatory and remains a personal choice:
\myinlinequote{And when we close the issue, it is not mandatory to document what did you do or create these kind of examples. I think that's something more personal decisions...We don't have that process integrated in our system. So me personally, I know from experience that this is really important so I do it.}
This sentiment was echoed by Subject 11, who emphasized the need for standardization:
\myinlinequote{I think firstly maybe you have to standardize what you should write.}
\DA{This is repeated for lessons larned documentation, should be removed here?}
When asked about documentation practices for lessons learned, \SubjectSix admitted that they rarely occur:
\myinlinequote{Oh, I don't think they are documented, pretty much at all. No, I think that there should be more a formal process at least on how to do that.}
Even when documentation does exist, there is no defined process for ensuring consistency, as \SubjectThree noted:
\myinlinequote{Yes, it might be, but it's not like there's a process for that.}

Half of the participants (5/10) described various methods used to capture failure knowledge, highlighting that such \ul{knowledge is distributed across multiple platforms and lacks standardization.}
\DA{A lot of quotes from here are also in lessons learned documentation, should be redone here.}
According to all participants, GitLab is the primary tool for storing failure knowledge. 
However, other tools and locations are also used, leading to fragmented documentation. 
The most senior participant (\SubjectSeven) shared that failure insights are sometimes recorded in formal scientific documents:
\myinlinequote{Sometimes...I'm writing down in some scientific documents...[and] publications showing the lessons learned... [and] white papers on ideas what's going wrong and what could be better.}
Another participant (\SubjectFour) echoed this sentiment, emphasizing the benefits of the publication process in uncovering issues:
\myinlinequote{Thanks to the publication process...we discovered some issues.}
Several participants highlighted that merge requests also contain failure-related discussions, as \SubjectFour noted:
\myinlinequote{There are also discussions in the merge request.}
Wikis were mentioned as another documentation method, though their use varied across teams. 
\SubjectTwo described how some teams create wiki pages and attach meeting slides:
\myinlinequote{Maybe in a sort of minutes of the meeting because usually we create a wiki page for such a meeting and we take notes...Usually the people reporting may have a few slides also they attach to this wiki page.}
However, not all projects have a dedicated failure knowledge wiki, making this approach inconsistent:
\myinlinequote{Really, when you look to the wiki page called ‘lesson learned from project,’ it's a few, not every project has one, but that’s the way of taking notes on a wiki page.}

Beyond the lack of standardization, participants also expressed \ul{confusion over where failure knowledge is stored}, making it difficult to retrieve and reference past failure knowledge and lessons.
\SubjectFive expressed uncertainty about where different types of failure-related information are stored:
\myinlinequote{I knew that there is a GitLab, but I didn't know what was documented in GitLab, what was documented in the wiki, what was documented on the team side, and what was discussed in which meeting.}
\SubjectFive further explained that where an issue is recorded depends on its scale and significance:
\myinlinequote{So if it's one of those bigger issues with the architecture, then it might get its own GitLab issue. Or if it's big enough to be discussed in the meeting with the other institutes, then it gets in the meeting notes. If it's just a local discussion focused on a single application or something, then I don't think it gets documented.}
Some participants confirmed that issues and lessons learned are not systematically stored. 
When asked about storage practices, \SubjectTwo stated:
\myinlinequote{Again, they're not really stored, they're just presented.}
When documentation does exist, it is often in informal formats, such as meeting notes or wikis, as \SubjectTwo explained:
\myinlinequote{At best, they are just on a wiki page.}
\DA{Repeated in lessons learned documentation. Part of it can be there and part can be here.}
The most senior participant (\SubjectSeven) mentioned contributing failure knowledge to a software engineering network within the organization, but this resource was not referenced by any other participants, suggesting low awareness or usage:
\myinlinequote{Today I would use wiki. Yeah. And I also share my experiences inside wiki. We have the software engineering network and several lessons learned inside the software engineering network coming from me with my experiences also.}

\myparagraph{Transferability} 
The pilot study confirms the case study findings that failure documentation and discussions are informal, ad hoc, and lack standardized processes. Participants described fragmented knowledge storage and difficulty retrieving useful information. For example, \PilotSubjectOne noted documentation was centralized in Confluence but still challenging to utilize: "\emph{you can search around...but it's hard to actually get stuff you can sit down and read}" (\PilotSubjectOne). Similarly, \PilotSubjectTwo explained postmortem information was captured informally as meeting minutes without structured templates, stating, "\emph{it just goes as meeting minutes...there isn't a specific template for the postmortem data}" (\PilotSubjectTwo). Additionally, \PilotSubjectThree emphasized personal discretion in documentation practices, reporting, "\emph{I think I was the only one who would document such a thing...}" with others leaving documentation to individual initiative.

However, transfer interviews also provided additional insights into practices for structured postmortem meetings, which occasionally occurred following significant incidents. For instance, \PilotSubjectFour described structured root-cause analysis meetings after production outages, highlighting formal methodologies like Six Sigma and "\emph{five whys analysis}" to identify root causes systematically. Despite these more formal efforts, the broader pattern remained informal and dependent on individual willingness or resource availability, as illustrated by \PilotSubjectOne, who explained, "\emph{we're very short staffed...we don't have time to write new people documentation}," underscoring a gap between ideal and actual documentation practices.

\subsection{Theme 2: Failure knowledge transfer practices are unstructured} 
All case study participants reported that failure knowledge transfer practices are unstructured and occur on an ad hoc basis.

\ul{Failure knowledge is shared through informal conversations rather than structured processes within teams.} 
\SubjectFour described how failure knowledge is shared through casual interactions rather than formal reporting, \myinlinequote{I will say that not officially, but it is common that during the day I discuss something with my team members, like my office mate or something like that, but not in an official way.}
\SubjectNine corroborates, \myinlinequote{Yeah, yeah, it's more like just Okay, just on the go.}
\SubjectFive reinforced the ad hoc nature of internal knowledge sharing, explaining that engineers typically communicate issues only when they need assistance, \myinlinequote{So if you have an issue, you basically tell the other people in your team that you have an issue, what exactly the problem is. Depending on if you expect them to help you or not, you can go into detail or not. And if they have an idea or if they encountered that issue before, then they will tell you. And maybe you make, if you have one person who says, 'Okay, I know how to deal with it,' then you can make a follow-up meeting with just that person. So you don't need to discuss it with everybody. I think that's more or less how it goes most of the time.}
A few participants reported that stand-up meetings provide a space to share obstacles and failure knowledge, but this is inconsistent across projects. 
\SubjectThree described the variability in this practice, \myinlinequote{Stand-up meetings where...discussing...obstacles...the discussion is to know also, okay, what if someone has had the problem before or if someone has an idea how to solve the problem. So this kind of communication, but it's not in every project.}


\ul{Failure knowledge is rarely shared beyond the immediate team, and there is little formalized communication across teams.} \SubjectOne noted that failure reports in broader project meetings are uncommon and often met with disinterest, \myinlinequote{Very rarely we report in a bigger round for the project that we experienced a failure or a problem and that we fixed it...the interest in that is also very low...So it completely stays in the team and will not be exchanged with others.}
When asked whether failure knowledge is shared to prevent mistakes from recurring in other projects, \SubjectTwo emphasized that it depends on the severity and relevance of the issue, \myinlinequote{I mean mainly depending on the criticality and relevance, I say it is clearly, if it's relevant for other projects or a very critical situation, then this information is spread in the group...we are trying to overcome it this way.}
\SubjectFive echoed this sentiment, explaining that engineers avoid sharing minor issues externally to avoid unnecessary meetings, \myinlinequote{You don't want to bore all the 20 people from other institutes with something that is probably not relevant for them.}
\SubjectThree explained how knowledge transfer occurs across projects, \myinlinequote{Within the project...Well, it depends very much on the project, how it's organized...let's say I work in one project, get some experience with certain part of problems, start working on another project, and of course I bring this experience with it and try to communicate this.}
Some participants mentioned that failure knowledge is occasionally shared in Brown Bag Lunch (BBL) meetings, though these are sporadic rather than regular practice. \SubjectTwo stated, \myinlinequote{BBL [Brown Bag Lunches - lunch and learn] meeting actually this sporadic one, not regular one.}


All participants mentioned that the primary method of \ul{failure knowledge transfer is through senior members mentoring junior members.}
The most senior team member, \SubjectSeven, was frequently cited as the go-to person for resolving issues.
A junior engineer, \SubjectNine, described their reliance on \SubjectSeven, \myinlinequote{In the beginning, till I get a better feeling for it, I would always check with [\SubjectSeven], 'Hey, how would you do it? Do you have any experience? What's the common way? What's best practice?' Yeah, that's the approach.}
When asked how past failures are avoided, \SubjectNine added, \myinlinequote{Yeah, but I also have to ask [\SubjectSeven] for examples} and \myinlinequote{he sharing his experience and we can then decide how we want to avoid problems or how we want to improve something.}
\SubjectSix described how knowledge transfer is largely dependent on direct interactions rather than documentation, \myinlinequote{Basically the way is...I have this issue...I could just go to [\SubjectSeven's] office and ask, okay, we have this issue, how would you tackle it? What do you think?...But yeah, normally it's just knocking at the door and asking, 'Hey, do you have any experience on these type of things?'}
\SubjectFive stated that this informal system works well for now, \myinlinequote{A lot of it is communication because we have some really experienced developers in the team. So when I have an issue, I usually...try to ask the people that are more experienced, and until now, that worked pretty well.}
\SubjectThree talks about the importance of this, \myinlinequote{Yeah, there should be [direct knowledge transfer], I mean that's how you grow as a developer, right? By getting maybe some influence by some similar experience.}
While senior engineers play a critical role in knowledge transfer, \SubjectOne noted that this approach can lead to inefficiencies in resolving recurring failures, \myinlinequote{A couple of situations which we had in the last couple of years where issues in our software popped up and sometimes they were recurring...So we experienced that someone was working on the software and he didn't fix it and he asked someone else on the team. And this one then said basically, 'Oh yeah, I remember that I faced this too. You have to do this and that.' So that's probably the worst case, how to handle those things, but that's how it was done actually.}
They also highlighted the difficulty of obtaining insights from past failures with such practices, \myinlinequote{It's like you have to hope and demand for this knowledge, so you have to ask other people if they experienced that and you got to hope that someone already experienced it or not.}
They say, \myinlinequote{This could happen only if the person who either fixed it or who was there in the discussion with members. I never experienced that, to be honest, that someone says like, oh yeah, we had this issue before and we fixed it like this and this and we can do it, but there's not a process to look it up to.}
\SubjectEight shares a similar drawback, \myinlinequote{its on the fly...if we or anyone sees something, it is shared, maybe you can do this in this way and you can avoid this,} and otherwise it's not.

\DA{New quotes:}
\SubjectTwo says, "The best way you need something that actually really bring you the lesson learned to the project mainly is coming from seniors working on the project. Usually they give you some hints from the beginning maybe to do that and not to do that and explain you why actually and what's the best way to do it and this what the best way not to do it. But when the project is done, as I said after wiki, then it's just gone."
\SubjectSix shares an example instance, "by senior members on the team like [team member] or [team member] for example, who is also sometimes helping us and there are constant reference by them, oh [in past project] this was done this way maybe should done this way. And I see there is always reference to these things" rather than looking at past failure knowledge documentation.

Although subjects admit the importance of ad hoc transfer of failure knowledge from experienced members, as \SubjectTwo notes \myinlinequote{they have all the lessons learned in [their] mind,} subjects also noted that \ul{sharing of failure knowledge should be integrated into training} to ensure that lessons learned are retained and systematically transferred.
The most experienced member, \SubjectSeven, emphasized the importance of mentoring junior engineers and passing down lessons learned, \myinlinequote{This is then more than a training issue. I think experience from the old colleagues must be also taught to the new ones, and it's also one of the reasons why [Team Lead] put me most of the time also in new projects and so on, so that I can share my experience.}
They also actively encourage junior engineers to reflect on lessons learned, \myinlinequote{Working together then with colleagues and also, yeah. Okay. Then teaching them and so on...I also request them, `Okay, what do you think? What was going good? What was going bad?' and so on.}
\SubjectFour described their approach to documenting lessons learned for training purposes, \myinlinequote{as a more senior member and mentoring younger members...I realized I have to explain again and again and again why I did that. So it's better to document that. And I noticed that the, they were doing something similar [mistakes as] when I started..., so I like to document the important fixes with examples and some documents that explain how the examples were and why the examples were in that way. I use that for training.}
However, this is not common practice and is often varied in practice.
\SubjectTwo says but is not done often, \myinlinequote{We save the problem...[and] sometimes lesson learned before and those are referred when someone new join...but again, that means it's not too often...The last time we referred to some reason was already two years ago or something.}
\SubjectOne says that \myinlinequote{we don't have a lessons learned page or database or something like that, which we guide them to.}
\SubjectNine, one of the newest members, corroborates this saying, \myinlinequote{No, as a newcomer for me, I wouldn't know. So it's not written anywhere, it's just the experience from the senior developers.} when asked if past documentation or advice is provided about past issues to learn from, and confirmed by \SubjectTen another new member, \myinlinequote{probably not as actively aware of.}

\myparagraph{Transferability}
The pilot study expands upon the case study's conclusion that failure knowledge transfer practices remain largely informal and unstructured. For instance, participants from the pilot study similarly highlighted senior-to-junior mentorship as a primary, albeit informal, transfer method, echoing earlier findings. One participant emphasized the need for more formalized mentoring structures, noting that mentorship currently depends on junior engineers proactively seeking knowledge: "\emph{They don't really incentivize that... it's more on the younger engineers to ask for it}" (\PilotSubjectOne). Additionally, participants reinforced the limited role of formal training, stating explicitly that failure knowledge is "\emph{out there, but it's not specifically addressed}" (\PilotSubjectFour) and new hires typically learn by observing experienced team members rather than through structured sessions: "\emph{they just watch how other team members are responding}" (\PilotTeam). These additional insights confirm the earlier case study observations about the ad hoc nature of knowledge transfer, while underscoring the broader need for systematic training and documentation processes to ensure effective learning from past failures.
%ADDITIONAL QUOTE NOT INCLUDED
%



\subsection{Theme 3: Learning from failure practices are unstructured} 


A paragraph about:
All subjects share that their failure management process ends with discussion and documentaion of resolution of issues, and rarely extends to preventing them or gathering lessons learned. 
Quotes are under codes: 
1. Failure is discussed upto initial fix (~prevention or lessons learnt)
2. Failure is documented upto fix (~prevention or lessons learnt)
...
These experiences show that the organization primarily applies artifact theory to identify contributing factors of failure as a part of their structured process. 
Although there are experiences shared applying systems-theoretic theory in ad hoc ways.
\DA{Reference to background section.}
\DA{Reference in discussion -> they seem to benefit from doing systems-theoretic in unstructured ways, maybe they should incorporate into their failure management process.}

\JD{An introductory summary like you did for Theme 1 and 2 would be nice.}
\subsubsection{Theme 3.1: Learning from failures lacks a standard process}
All subjects share that there is \ul{no structured process to learn from failures}.
When asked whether formal efforts exist to prevent repeating mistakes, \SubjectFive stated:  
\myinlinequote{I don't think that we have a formal process on how to make sure that it doesn't happen again.} 
Similarly, \SubjectSix confirmed that reflecting on and preventing failures is not a standard practice:  
\myinlinequote{This rarely will occur. I have never been in a situation like that. I guess this will happen...we don't have a very strict process for that, to be honest. Not really.}  
\SubjectNine was also unsure about whether such a process exists, deferring to a more senior engineer:  
\myinlinequote{But I actually don't, I know it happens, but actually I think \SubjectSeven can tell more about this. Yeah, if you want to have any examples, maybe ask him for this. He has a better overview.}  
\SubjectThree confirmed that reflection and group discussions on failures do not happen systematically:  
\myinlinequote{It's not that much that there's a big reflective period where we say, okay, this error happened and now how should we do that now in the future...it's not, so the reflection part that you come together as a group and let's say now reflect on the bug you notice or something is usually not part of the things.}  
\SubjectFour attributed the lack of reflection to the nature of their development approach:  
\myinlinequote{Yeah, because we are not following this totally agile approach...that process, no, we don't do that...usually in this kind of space project you don't see total agile.}  
Although they expressed interest in implementing such a process, they acknowledged that it is not currently part of their workflow: 
\myinlinequote{I would like to, but I think at least my project is not the case. Got it. Okay. Yeah, I like the idea, but we don't do that.}  


While structured reflection does not occur consistently, some participants described \ul{sporadic or informal efforts to discuss lessons learned}.
For example, \SubjectEight described an upcoming meeting to discuss lessons learned, but emphasized that this is not a standard practice:
\myinlinequote{No, I can't recall [if we've done one before, but]...we're going to do this actually in a couple of weeks...but...No No, it is not standard. Yeah, it's not standard, but I think it's a good way to see how we can improve.}
They also noted that while their team is planning to discuss process improvements, this is a one-time event rather than a recurring practice:
\myinlinequote{We are going to discuss about the process. At least I have some feedback from that, how we can improve what are maybe kind of our bottlenecks during development.}
One of the newer subjects, \SubjectNine, contrasted their current workplace with a previous organization, noting that while failures are addressed informally, there is no structured learning process:
\myinlinequote{We do it quite more often and on the fly...we are more open to adjust and change the code to make it improve it on every step and not fixed structures at which milestone you have to do this. But negative point is of course that there's no real structure -- It's more like sharing experiences.}




When it does occur, \ul{learning from failures is  driven by personal motivation rather than a structured process}. 
\SubjectFive noted that improvements happen because individual developers take the initiative, not because of a formalized effort:  
\myinlinequote{I gave...feedback...so now there are some improvements being made...But I guess those steps that are being taken are not in a process defined by itself, but they are more on the personal motivation of some developers.}  
Similarly, \SubjectFour described how learning from failures is not mandated but rather left to individual discretion:  
\myinlinequote{I don't think it's something mandatory because, yeah, no, nobody told me specifically to do that, but I think those are general good programming practices...I try to implement those kind of good practices like documenting the issues, learning from them to reflections about that, but not as something actually part of the main software development process.}  
They further emphasized that adopting reflective practices is a personal choice rather than an organizational expectation:  
\myinlinequote{I think that it could be up to you to embrace these practices and actually applying where you are working. And I think that's something that you can differentiate between good programmers are programmers because you notice these kind of practices.}  


Participants described \ul{certain heuristics influence when learning from failures occurs}, often based on the perceived criticality of the issue, if its due to system architecture or development processes, and review requirements.
\SubjectTwo noted that whether issues are formally studied depends on their criticality, particularly the potential damage or delays they might cause:  
\myinlinequote{Issues are studied and lessons learned gathered based on criticality [determined by potential] damage or the delay may cause to solve the damage.}  
In some cases, structured failure analysis is required by external standards as \SubjectTwo highlighted, 
\myinlinequote{For some projects, if you look to the standard the European Space Agency, you'll see a review plus one to actually collect lesson learned...But this doesn't apply for all of our projects and I don't know actually in this project how much serious they are with this review.}  
\SubjectFive explained that discussions on preventing recurring issues generally only happen when the failure is architectural:  
\myinlinequote{Only if it's a structural problem, if it's a problem with the architecture or something that everyone will have to deal with at some point.}  
Similarly, \SubjectSeven stated that software failures are rarely examined systematically, unless they reveal a broader process issue. 
When asked if there's a process to gather lessons learned, \SubjectSeven says, 
\myinlinequote{Not really. It's a software failure most of the time. Yeah. But for me, okay as always case was it only in think what I didn't see or was it something wrong in the process or so on when something wrong it's in the process then okay, then maybe such process or modification of the process of your development processes.}  
Rather than focusing on software-specific lessons learned, \SubjectSeven mentioned that reviews tend to emphasize project-level insights from past experiences,
\myinlinequote{Normally when you review the first time a new project plan...from this management setting, it was the experiences, what's going from and projects and so on.}  
However, even this form of reflection is not systematically reviewed within the department:  
\myinlinequote{This is not reviewed by this department.}  



Many participants highlighted that the \ul{absence of a structured process results in recurring failures}, as past mistakes are not systematically reviewed, and expressed a \ul{desire to implement a process to learn from failures}.
\DA{Repeated quote here - but it fits better here}
\SubjectOne described how recurring issues remain unresolved due to inefficient knowledge transfer:  
\myinlinequote{There were a couple of situations which we had in the last couple of years where issues in our software popped up and sometimes they were recurring, so sometimes I saw them again and again, but there wasn't actually a process how to handle those. So we experienced that someone was working on the software and he didn't fix it and he asked someone else on the team. And this one then said basically, 'Oh yeah, I remember that I faced this too. You have to do this and that.' So that's probably the worst case, how to handle those things, but that's how it was done actually.}  
\SubjectEight recognized that teams handle learning from failures in their own way, and suggested that a unified feedback process could be beneficial
\myinlinequote{Actually, I don't know. Okay. I don't know. Yeah, I think some kind of feedback is needed, but I think every group is dealing with this in their way. It's like we don't have a process.}  
Similarly, \SubjectFive acknowledged that while the organization has processes for many aspects of development, having a structured process for learning from past mistakes could save significant time and effort:  
\myinlinequote{Not as far as I know...I mean, we have processes for everything and I guess it would be helpful to have a process to learn from mistakes regarding code quality because it probably takes a lot of time if people make the same mistakes over and over again.} 
They also suggested that integrating a structured learning process within employee onboarding and training could be beneficial:  
\myinlinequote{I feel like a process somewhere embedded in the onboarding process of new employees would definitely help.}  



%They also mention, \myinlinequote{we have once a year...where the different groups of the department meet with some purposes... and there is some exchange of ideas}


\subsubsection{Theme 3.2: Lessons are gathered inconsistently}

Most subjects (8/10) from the case study share that \ul{lessons learned are gathered in an ad hoc and informal manner}, often relying on spontaneous discussions rather than structured practices.
For example, \SubjectTwo described how gathering lessons:  
\myinlinequote{It's more on the go...their lesson learned,...it's mainly up to the group level, like the group leader and the seniors on the group.}
\SubjectSeven, the most senior participant, described: 
\DA{Repeated but may fit better here}
\myinlinequote{Normally for me it's always necessary after a project to do going inside and checking what's good, what was wrong, what would be better and so on.}  
They also noted that they sometimes initiate informal reflections with collaborators:  
\myinlinequote{In some projects, I request [from collaborators], okay, what do you think? What was going good? What was going bad and so on.}  
Similarly, \SubjectSix provided an example of gathering lessons learned for the next version of a project:
\myinlinequote{Let's say we kind of sit down together and we brainstorm or we already had a list [of issues], right? Okay, these are the things we have...this is how it went, this is how it works. Overall it went well. So it was a success, but there are these and this which could be improved.}  
When asked whether this practice was formalized, they clarified:  
\myinlinequote{No, I don't think we have a very formal standard process, at least in our group. Yeah, I mean we are mostly a research institute and we are not a software house, but we don't have very standardized processes or ways to do these things.}  
\SubjectTwo reflects that gathering lessons learned occurs at varying frequencies:  
\myinlinequote{Not every day, not every month, not every year maybe. It depends on the project in which phase it is...usually at the end of a project. So maybe you report about the project and then study lesson learned about the project. Sometimes...at some milestones of some reviews... sometimes you don't have much things actually to study.}  

Several \ul{participants struggled to recall specific instances where lessons learned were gathered}.
For instance, when asked to recall a time they studied a failure to gather lessons learned, \SubjectFive admitted:  
\myinlinequote{I actually thought quite a while about that and I can't really find a single example for that...I can't think of a single time where we just sat there and discuss...issue to avoid it in the future.}  
Similarly, when asked if they had been part of a meeting to discuss lessons learned, \SubjectNine stated:  
\myinlinequote{No, not that I can think of, no.}  
\SubjectThree reported holding dedicated review meetings to reflect on lessons learned but can't recall instances of such meetings except after a satellite launch:  
\myinlinequote{I try to do this basically on a regular basis in the review process of development that we have a dedicated, let's say appointment just for that...Don't remember too much except for as after a satellite launch, then of course there was, but then the lessons learnt may not just regarding development, but the whole project.}  


Half of the subjects seemed to think that discussing a failure or fixing a problem was the same as gathering lessons learned, revealing a \ul{misunderstanding of what constitutes a learning process}.
For example, when asked how they learn from failures, \SubjectTwo described discussions about problems and verifying solutions:
\myinlinequote{[We] follow this obvious structure that you show the problem and you show your approaches such [as] this problem. What was your solution, what you tested, what you studied already, what was the conclusion of that? Sometimes of course it'll be a sort of a discussion way that you say, okay, didn't, why you didn't test that option, what would be the case? So then it'll not to bring the lesson learned immediately, but more to discuss the problem and verify the solution let's say.}
Similarly, \SubjectSix assumed that identifying and documenting a solution to a problem was equivalent to gathering lessons learned:
\myinlinequote{Well, both the issues were kind of the lessons learned and then they describe, okay, no, but actually not, it's not. It's more will be more, okay, there was this issue and then the lesson learned will be, okay, we need to fix this issue. So then we created an issue with the title..., and then this is a bug, they should be fixed this way.}
When probed further about what exactly is captured in the lesson learned documentation,\SubjectNine described capturing only general descriptions of the issue and solutions:
\myinlinequote{Yeah, the experience I...[have, it's] just a general description of the issue and what the suggestions were. But overall pretty general.}
This misunderstanding extended to postmortems as well. \SubjectTen describes, \myinlinequote{every two weeks we have a scrum meeting and we do speak about the things once they are finished. So we speak about the plans we have for the future but also the things that we have finished or are working on. So if this counts as a postmortem meeting, then I would say that was the time when we told our colleague about changes, so that maybe counts as postmortem.}
\SubjectFour assumes that creating example code to reproduce issues and is enough to prevent recurring failures:
\myinlinequote{what I do is to create examples, example code examples to reproduce the issue to document the issue and add this example to the continuous integration system. So we are sure that this issue is not going to happen again.}







\subsubsection{Theme 3.3: Lessons are documented poorly}


Half of the participants described that \ul{lessons learned are documented inconsistently}.
Subjects reported documenting lessons learned in fragmented ways. 
\DA{Quote is repeated, but there's another quote that could be switched in: "So that I have also there are some publications that showing the lessons learned"}
For example, \SubjectSeven shared that they sometimes document lessons learned through scientific documents or white papers:
\myinlinequote{Sometimes yes and some scientific documents that I'm writing down...is lessons learned from the previous project...and writing also white papers...on the ideas what's going wrong and what could be better.}
Additionally, \SubjectSeven mentioned using a wiki to document lessons learned:
\myinlinequote{Today I would use wiki...[to] share my experiences inside wiki. We have the software engineering network and several lessons learned in inside the software engineer network coming from me.}
However, no other participants referenced this wiki, suggesting that it is not widely known or used\JD{This wiki thing is great and a good example of why case studies are nice. Please don't cut this story. But I'm confused because you say S2 also refers to a wiki. Same wiki?}.
Some subjects described capturing lessons learned in project documentation, albeit in a broad and sometimes ineffective manner. \SubjectNine shared that lessons learned are documented at project milestones but described the content as general and lacking detail:
\myinlinequote{I know we document lessons learned in the project phases. I think it's happening at the end of every milestone or so...it's more like the whole project than for the software development. I'm not sure if something like this [for software] exists.}
When asked what this documentation includes, \SubjectNine clarified:
\myinlinequote{Just a general description of the issue and what the suggestions were. But overall pretty general.}
\DA{Repeated but better fit here}
\SubjectTwo also described a common ad hoc practice of documenting lessons learned within meeting minutes or wiki pages, but emphasized that this is not a consistent practice:
\myinlinequote{Not always. Maybe in a sort of minutes of the meeting because usually we create a wiki page for such a meeting and we take minutes notes, maybe not really minutes, but notes on that...Really when you look to wiki the page called lesson learned from the project, it's a few, not every project has one, but that's the way of the taking notes on a wiki page...but that's actually not standard, not always.}


In contrast, half of the subjects indicated that \ul{documentation of lessons learned are often omitted}.
When asked directly if lessons learned are documented, several participants confirmed that they are not. \SubjectFive stated:
\myinlinequote{Not in the project that I've worked with so far.}
Similarly, \SubjectTwo said:
\myinlinequote{We track issues, but yeah, not for lesson.}
\SubjectOne confirmed that no formal system exists for recording lessons learned:
\myinlinequote{We don't have a lessons learned page or database or something like that.}
Even in cases where teams conduct reflective discussions or meetings, documentation is often absent. 
\DA{Repeated, but connected - remove the documentation part from previous occurance}
When asked whether the lessons learned from the organization-wide meeting on software practices will be documented, \SubjectEight responds, \myinlinequote{No, I think...probably we'll take notes. Not sure if there will be a minutes taker or something. I don't think so really, but probably, I mean everyone is taking notes.}
\SubjectSix similarly described that general (not just software) post-mission debrief meetings were sometimes documented, but detailed lessons learned were rarely recorded:
\myinlinequote{So this general meeting was documented with general minutes of meeting...[Lessons learned?] Oh, I don't think they are documented, pretty much at all. No, I think that there should be more a formal process at least on how to do that.}
The lack of documentation has resulted in knowledge loss, as described by \SubjectTwo:
\myinlinequote{Actually this knowledge could be lost because they are not well documented and not well processed to transfer it in a process...somethimes [we] forget that one and then actually it's gone because there's no process to say no, part of your project is to write lesson learned.}
\SubjectOne admits the process to document lessons learned is unknown, \myinlinequote{How to document learnings, that is probably something also, this is a hurdle. How do we document that?}


\DA{We could pull in some quotes about how subject 7 internalizes a lot of these lessons learned.}

Subjects indicate that \ul{lessons learned are internalized rather than explicitly documented}. 
When asked if lessons learned are documented, \SubjectTen stated:
\myinlinequote{No really lessons learned, no. I think they're more like internally...we learned from it.}
\SubjectEight similarly described that while they recognize common lessons or risks, this knowledge remains informal and undocumented:
\myinlinequote{I mean just from implicit, not explicit, but implicit. Okay. I know that some kind of pattern or doing the thing in some way could be dangerous and you learn how to do it in a better way, but this is just internally knowledge you're learning. But yeah, I'm not like if I, for example, document how I implemented the issue...[or lessons] No.}
In some cases, even when recurring issues are discussed, their lessons learned are not formally recorded. 
\SubjectTen described a discussion about a recurring problem, but admitted:
\myinlinequote{It was more just a discussion I would say. I think there wasn't an active writing down, 'let's not do this again.'}
Other participants shared similar experiences. 
When asked if lessons learned are documented, \SubjectTwo responded:
\myinlinequote{No. No. Do not see lesson learned. You'll find the discussions [in issue reports,] but not explicitly referred that this is lesson learned from this project.}
\SubjectTwo adds:
\myinlinequote{They're not really stored, they're just presented...best way, they are just on a wiki page.}
\SubjectSix described a recurring problem and admitted that documentating lessons learned would be beneficial:
\myinlinequote{I don't think we document it anywhere to be honest. No, I don't think so. Maybe it would be a good idea.}







\subsubsection{Theme 3.4: Lessons are applied ad hoc}

About half of the subjects say that failure knowledge is reviewed later, and about half of the subjects say that failure knowledge is not reviewed later. 


Group 1: Referencing Past Issues is Inconsistent and Often Relies on Individual Initiative
2. Learning from Past Incidents Often Occurs Informally Through Discussions Rather Than Structured Processes
3. Lessons Learned Are Sometimes Captured in Project Documentation, but Such Documentation is Rarely Referenced
4.  Some Teams Attempt to Apply Lessons Learned Through Specific Design Changes or Process Improvements
5. Some Participants Assume That Learning from Failures is Handled by Others, Leading to Gaps in Practice
6. Some Participants Assume That Learning from Failures is Handled by Others, Leading to Gaps in Practice



Several subjects mentioned occasionally referring back to \ul{past issues to help solve similar problems}, but this practice is informal and dependent on individual initiative rather than a structured process. 
\SubjectFive explained that they occasionally revisit past meeting notes or issue reports when encountering familiar problems but emphasized that this occurs infrequently:
\myinlinequote{The issues...appear over and over again. If you check the open issues, the meeting notes are not really checked. Again, only if somebody knows that there is something interesting. But usually I think I've looked into old meeting notes maybe twice or three times.}
Similarly, \SubjectTwo briefly noted that they also reference past issues on occasion:
\myinlinequote{Sometimes yes.}
\SubjectThree described relying on closed issues to help resolve similar problems but noted that this practice is informal and not integrated into a structured learning process:
\myinlinequote{What I have done a couple of times is actually then search through the issues, even the closed ones, to figure out, okay, remember I had this kind of problem before, so maybe I can find what I did last time,...but it's not in the process...to prevent...these issues again.}
\SubjectTen similarly shared that they often reference closed issues to understand how previous problems were resolved, but emphasized that this is a personal practice rather than an organizational norm:
\myinlinequote{very often what I do is I search in GitLab or GitHub closed issues to see how they solved something...I don't know if other people do it.}




Some subjects described \ul{learning from past incidents through informal discussions}, such as team meetings, coffee breaks, or ad hoc conversations. 
While these discussions sometimes result in useful insights, \ul{they are not systematically shared}. 
For example, \SubjectTwo  described informal discussions occurring during casual conversations rather than dedicated meetings. 
As \SubjectTwo noted,
\myinlinequote{Yes, they are...even sometimes in coffee break...Oh yeah, actually, we had this issue and we tried to learn this...Then you may be involved in short discussion...so I learned from their lesson learned, then I personally will keep it in mind and try to implement or come to them when I face a similar problem.}
\SubjectTwo also describes how in some cases senior team members may share insights during team meetings, but these insights are often not formalized or widely disseminated:
\myinlinequote{One or more senior people...when they figure out measures to avoid it, then in our pre-weekly meeting they diagnose it and maybe they will schedule a recent round table or a meeting to actually explain the problem and how they overcome it...People will look into it. Sometimes even the people will not look and they face the problem again later.}
\SubjectTwo further highlighted that referencing past knowledge is often driven by memory or informal conversations rather than structured documentation:
\myinlinequote{If no one gives you the link, usually you cannot find it... [It's more] "Oh, I saw this before somewhere." Unless you know that this project has a wiki page or a page, then I will visit and check. Because you had previously [knowledge] that they discussed this problem in that product or you call a colleague and say, okay, you are working on their project. I heard about this.}
However, when asked if past issues are referenced, they say, \myinlinequote{Not really.}


While some participants noted that \ul{lessons learned may be documented in wikis or other repositories, but are infrequently consulted and are inconsistently integrated into development}. 
\SubjectSeven described using wikis to document insights from past experiences:
\myinlinequote{Today I would use wiki...[to] share my experiences inside wiki. We have the software engineering network and several lessons learned inside the software engineer network coming from me.}
However, no other participants mentioned consistently referring to lessons learned from such wikis, suggesting that these resources are not widely referenced. 
In fact, \SubjectOne explicitly stated that past issues are "unfortunately not" referenced. Similarly, \SubjectEight confirmed that referencing past documentation is not common practice:
\myinlinequote{No, I think it's not so.}
In some cases, participants believed that documentation existed but were unsure if it was actually utilized. 
For example, \SubjectNine mentioned that lessons learned are sometimes saved but noted that this occurs infrequently:
\myinlinequote{We save the problem...[and] sometimes lesson learned before and those are referred when someone new joins...but again, that means it's not too often...The last time we referred to some reason was already two years ago or something.}




A few subjects shared examples of \ul{technical or process improvements that resulted from past failures}. 
However, these improvements were often reactive, occurring only after issues reoccurred or through individual initiative rather than being part of a structured learning process. 
For example, \SubjectSeven recounted an incident where a critical configuration error lost control of a satellite launch:
\myinlinequote{This was a big fail for the team...the project manager called me by phone and I hear it from the sound of his voice there was crying and yeah, yeah, everything is not working...we cannot start the satellite...[because of incorrect] configuration management...They going into the wrong directory working on the three-month-old software version and nothing works...[during] the phone call, 'Yeah, I know this failure, this was fixed three months ago'...They recognize, okay,...[it's] the wrong software version...This was also one of the lessons learned and the reason why we have right now this modeling...group in our department and test process...[and] had a research project out of it...the loop testing approach.}
Similarly, \SubjectSix shared an example where their team applied lessons learned from one mission to improve the design of the next project:
\myinlinequote{From the results of mission one...we learn a lot of things...we are applying it for the new mission...it's a lot of lessons to learn that we extract from the post mission...or even during the mission...[this was done ad hoc by] oh, this could be done better, but we don't have the time to do it now, we do it afterwards, and now we have the time in between missions kind of implementing the changes...I was there to compile this lessons learned now implementing them in the next generation.}
%And when asked if the issues recurred after this, they respond, "No. Most of the time we were able to solve them effectively. Yeah.




Some subjects assumed that other team members were learning and addressing recurring issues. 
For example, \SubjectNine expressed hope that team members were capturing lessons learned but had no direct evidence of this:
\myinlinequote{Sure, yeah, definitely. I mean you don't want to repeat the same issues, but I don't have any example, but I hope [the rest of the team] are taking care of this.}

Although some participants mentioned the existence of \ul{tools like wikis or questionnaires intended to facilitate learning from failures, these resources were inconsistently used and often overlooked in practice.}
\SubjectSeven described a questionnaire designed to encourage teams to reflect on lessons learned:
\myinlinequote{There's a questionnaire to get them [to reflect on lessons learned].}
However, when informed that no other participants mentioned such a questionnaire, \SubjectSeven admitted,
\myinlinequote{Normally you should use it always when you set up a new project. As I say, normally... But some people they didn't do it...From the structure inside [the agency], we cannot do it that everyone has to do it...There's a template to do it, but it's not standardized to do it.}







\SubjectFour also says, "when someone is wondering how to design a new application, for example, we have a set of examples at hand, or if someone is having issues with the code, something is not working, we can show, oh, we already experienced that issue, so here's an example of how to do it. In that case cases, let's say both for training also and to guide...Yeah, yeah, I have done that...searching for similar issues in GitLab."



\SubjectNine says, "What we use is, for example, we have another project from the past which we're working really well and everyone was kind of happy with the outcome. So we used this example on how to implement our staff. So we thought, we always look at our project and see, okay, it was working quite well back then so maybe we try to do it the same way."


\SubjectSeven says, "in my first space project, they have the idea to make it cheap, so building by low income, good satellite and their solution was don't write documentation...This totally failed in my opinion, at least for me then [the lesson is that] at least these interface control documents are necessary."
\SubjectSeven says, "this tasking framework is also lessons learned from this first project"

\SubjectOne shares an example, "There were some things in the development...where we said, okay, that's something a lesson learned and we tried to fix that in the operating system...I think [fixed] in this operating system...But yeah, I think this [issue] occurred again, due to the fact that we at some point flashed the whole target again with a new operating system.  Yeah, we specific very specific problem, which occurred several times and yeah, not like that we said that's a process we need to follow, but that's like, okay, yeah, we might be able to change that in the operating system."
- Narrative: recurring issue that resulted in technical architectural fix, but was not documented, so it happened again when the architecture was reset?

\SubjectThree: "So we then let's say...[we have] errors areas can harm you and take very long to figure out. And then trying to make fair, safe afterwards that this at least doesn't happen. Not at the same place again, but also in general less often.  I mean we had several specific incidents where we had...not the same error, but the same type of error [reoccurred]. Yes, I think [we took measures to prevent recurrence]. At least in the follow-up project, I usually try to have a lot of checks beforehand to at least in the early part of the development process to figure out potentially dangerous things. So that's then later on you don't have as many pitfalls."

When asked if they have notices recurring issues, \SubjectEight says, "yes. I noticed something, for example, for starting a new repository, we need a structure, a common structure for this kind of different flight software...We figure it out in the team, we figure out that and start developing templates for this common structure"

When asked for an example of them learning from a failure \SubjectSix says, "Yes. I think we actually had a session not too long ago where we just came into the situation where we realized...that our [architecture] is doing more than it should, so it's not really well separated and it just became too big. And then we just looked at our initial idea and initial architecture. I think one of the reflection that was just you have to be really careful with [the architecture]. Every time I think of [it] now, I kind of think of the situation we were in before, so I think it made me more aware of the downsides I think."

When asked how often they actually refere back to past issues and lessons, \SubjectFour says, " I think that sometimes. Sometimes happens. Sometimes, yeah."

\DA{Maybe this goes to knowledge transfer? - If we decide to talk about transfer of lessons learnt knowledge, then we can grab more quotes from there to here }
\SubjectTwo: "So I think, and again, you'll be self-motivated to search the wiki, search the GitLab, ask the seniors, otherwise this no will not be, or there's no process to bring this lesson down to you."

\JD{The next part sounds like it is about tracking, not applying. But the rest after this big quote, that rest sounds like it fits Theme 3.4}
For instance, when asked whether there are discussions about how to prevent issues from recurring, \SubjectThree explained that while serious issues may prompt reflection, no structured process exists for capturing lessons learned in most cases:
\DA{Repeated quote, but can be orged to not be repeated}
\myinlinequote{It depends, right? I mean, if it's an issue that causes a mission to not worry, then of course there will be a full thing. If it's during this process of development, I would say no further action will be taken. And I guess it's more than part of the whole knowledge of the group of similar issue happens afterwards. Okay, this other issue we saw within this way, so maybe we can do it like that, but we don't have a formal way of keeping track... This rarely will occur. I have never been in a situation like that... Other than that, we don't have a very strict process for that, to be honest. Not really.}


\SubjectSeven shares an incident, "we lost control of the satellite....lessons learned for me for these situations [technical lessons]. This is discussed and then in the next designs we [applied technical lessons]."


\SubjectSeven says, "when I setting up a new software, I try to avoid this failure again" but when asked if this is standard, subject replies, "I can only say do this lessons learned process and normally I think it's also written down somewhere in our processes. But what I see it's most of the time, okay, we didn't have time, we need to set up the next project."



\DA{The following two may be more appropriate for knowlegde transfer?}

\SubjectTwo shares an example of ad hoc sharing, documentation, and integration of lessons learnt, "I remember when I joined...they were talking how to not do a thing again. I think that was ex-colleague was explaining what they faced and how they figure out how to handle the issue...then we talked about that we need that day there was the documentation was limited or poor...then we were talking that to improve the documentation but to define patterns and anti patterns." and "people who joined afterwards, they follow the same instructions...to not to make the mistake anymore and actually if I remember we didn't have a problem."
\DA{This can be referred back to when we talk about knowledge loss when people leave?}

\myparagraph{Transferability}
The pilot study aligns with the case study findings that organizations lack structured processes for systematically learning from failures, with discussions often limited to immediate fixes rather than long-term prevention. For instance, participants explicitly stated the absence of formal reflection processes, with \PilotSubjectOne admitting, "\emph{There's no process for that}," and \PilotSubjectThree confirming explicitly that, "\emph{No, we did not study the software failure itself}." Similarly, the ad hoc nature of failure resolution was clearly described: "\emph{they just hack their way through finding the bug and fix it}", aligning closely with the case study participants' statements, such as \SubjectFive's acknowledgment that "\emph{I don't think that we have a formal process on how to make sure that it doesn't happen again}." Both studies thus highlight a common lack of structured efforts to systematically learn from and prevent recurring issues.

Additionally, the pilot interviews provide insights into inconsistencies and misunderstandings around referencing and applying lessons learned. While some participants noted occasional structured meetings or documents, the utilization of these materials remained inconsistent and dependent on personal initiative or leadership style. For example, \PilotSubjectFour explained that postmortem outcomes depend entirely on "\emph{who's running [the meeting]}" and noted that recorded actions "\emph{get incorporated into any new development}" only if someone actively initiates follow-up. However, multiple other participants had different practices; \PilotSubjectThree and \PilotSubjectOne explicitly stated lessons were "\emph{not referenced once [the project] is closed}," suggesting significant knowledge gaps and misconceptions. These experiences closely align with the case study findings, indicating that lessons learned are either internalized informally or entirely neglected, leaving failure management practices largely ineffective.


\subsection{Theme 4: Recurring failures and the illusion of effective failure management}


All subjects report that there are recurring failures. 
%%
\DA{Repeated but most appropriate here?}
\SubjectOne noted inefficiencies in resolving recurring failures, \myinlinequote{A couple of situations which we had in the last couple of years where issues in our software popped up and sometimes they were recurring...So we experienced that someone was working on the software and he didn't fix it and he asked someone else on the team. And this one then said basically, 'Oh yeah, I remember that I faced this too. You have to do this and that.' So that's probably the worst case, how to handle those things, but that's how it was done actually.}

\SubjectOne shares another example of how a recurring issue was handled and how no steps were taken to prevent further recurrence, "someone called me and asked, here I have this and that issue. Have you ever experienced that? And I basically helped them, but further than that, we didn't take any measures to prevent that."

\SubjectOne:
"And there were a couple of situations which we had in the last couple of years where issues in our software popped up and sometimes they were recurring, so sometimes I saw them again and again, but there wasn't actually a process how to handle those"

All subjects report that there are recurring failures. 
\SubjectFive:
"The issues are quite often because they appear over and over again."
"I think in my current project, there are some issues that do occur again and again."

\SubjectSix:
"I see that we're kind of committing the same mistakes over and over just in different phases. But at the end it's the same thing."

\SubjectSix described a recurring problem and admitted that they did not document it:
\myinlinequote{we have had a situation where we had a problem, we thought we solve it, then we had another problem, we solve it and it was always the same problem all the way...I don't think we document it anywhere to be honest. No, I don't think so. Maybe it would be a good idea.}

\SubjectSeven attributes recurring failures to newer members, "I see that happened again and again because most of the young engineers, software engineers coming directly from the university, they didn't have the experience and the sharing of experiences is limited."
Another example, "the same problem...nasty. The same happens again. It always, you have always the same cycle and most of the times."


\SubjectNine says, "A few issues there probably...we have to face the same issues again instead of implementing it in a proper way and stuff like this."

\SubjectOne says, "And there were a couple of situations which we had in the last couple of years where issues in our software popped up and sometimes they were recurring, so sometimes I saw them again and again, but there wasn't actually a process how to handle those."

\SubjectOne recounts an example of an issue that they discussed, "And after a while someone forgot. And after a while this issue popped up in our queue again and we started discussing and we were like, wait, we discussed this already five months ago."

\SubjectTwo recounts an example, "the same problem but a different place because it's got a different project, different requirements, so similar problem but it just emerged from a different case."
%%


Disconnect between subjects thinking their failure management is working, except they report recurring issues.
%%
Subjects seem to assume that general software practices are enough to prevent failures often devaluing the need for learning from failures. 
When asked if they notice any gaps or opportunities to improve some of these practices, \SubjectSeven says, "There aren’t really gaps, there’s training. The only issue we have time to get the lessons and performing the lessons. That's why we have this on-boarding process."
\SubjectNine says, "we have kind of a structure there already...we have our requirements...we have a test driven approach...of course there are the guidelines, there are standards...I think that's the main points how that we know that our design might be good."
When asked if they study failures beyond its fix to gather lessons learned, \SubjectOne says, "No, usually it's for fixing the bug. I mean, when we consider patterns of things, we always have to take into consideration that we have a certain coding standard we need to apply. So we sometimes cannot move from certain patterns. I mean I never experienced that a pattern which is enforced to do by us causes some problems because those patterns are really wisely chosen, but we are not that free in choosing patterns there. But for your initial question, I would say no. We studied the problem in order to fix the problem and not in order to retrieve some knowledge out of it."
\SubjectThree says, "all the development is done with the peer review before it's merged into the main development branch...So you basically can there see, okay, we have certain coding guidelines which tries to do some defensive programming techniques to avoid certain kinds of errors from the get go. And there you can basically look and then do the review process. And in the beginning it might be that you open more discussions then with a more experienced developer...And of course then you can say, okay, please have unit test which create a certain amount of code coverage to figure out some common situations."
When asked about what they do to prevent recurring issues, \SubjectFour says,"we use several, many general measures to avoid these kind of things like following code standards, following product assurance standards, following, I don't know. And not only following, but we also have to report these kind of things. For example, when you are in this kind of a space project, you have to report the test cover. If you deviated from some rules, you have to explain why or probably you cannot deviate if it is not a good justification for that. So I think there is a whole umbrella, which is sometimes not fun because it's related with documentation, with following standards that prevents you from doing real or sometimes optimal things let's say. So this following these rules should prevent these kind of issues, but it's not always the case...I think that's the main thing. The whole standard and quality standards we follow... think that what really prevents you prevents that is following the process I mentioned."
\SubjectFour explains that much of the learning process has already occurred, and the lessons learned from them are established as standards and guidelines, so if they follow them, the need for ongoing reflection and learning is minimized:
"it is not that we are learning what to do, what we are programming, despite some issues as I mentioned before, because we know the criticality of our projects in advance and we know at least some general rules, standards, whatever, that we have to follow to prevent that and to deliver the expected product quality...[with these standards] we know in advance what things are dangerous for this kind of critical code. So I think this reflection process occur years before...and we already have that experience [as standards] and we are using this experience."
"Best practices, guides or standards coding a standard on product assuring standards because those standards usually collect years of experience in software development from." 
When asked about about their thoughts on a process for learning from failures, \SubjectSeven  assumes that only new members need to learn from failures, "So long the process is understandable for new employees...The new employees you're getting directly from the university didn't speak the language...So you think that it would be beneficial for new employees, but for experienced employees it might not be necessary...It's a big knowledge base normally"
%%

A few subjects (4/10) share examples where they learned from failures ad hoc and it did not recur. 
%%
\SubjectFour shares an example of learning from a failure, documenting, and sharing, the lessons as, "we have to define a guideline pattern on anti pattern, how to do it and what not to do next time to actually not get this problem anymore," and as a result the problem did not recur "because the people who joined afterwards, they follow the same instructions."
From \SubjectSeven's example of the incident the lessons learned were "discussed and then in the next designs when we have alway...[implemented lesson]...and no, [it has not recurred] as of yet."
After a recurring failure, \SubjectThree, "in the follow-up project, I usually try to have a lot of checks beforehand to at least in the early part of the development process to figure out potentially dangerous things...so you have your automatic pipeline, which tells you you're doing something wrong and then please fix it."
%%

\myparagraph{Transferability}
The pilot study agrees with the case study's finding that teams repeatedly experience recurring failures despite believing their failure management practices are sufficient. Participants openly acknowledged ongoing issues, with one explicitly stating, "\emph{we come across the same issues over and over again...the tech debt just gets rolled forward and it gets worse and worse}" (\PilotSubjectFour), closely echoing the case study participants’ frustrations about unresolved recurring problems. This parallels the case study’s finding where participants recognized issues repeatedly resurfacing but still lacked structured processes to prevent recurrence, as exemplified by \SubjectOne: "\emph{issues in our software popped up...sometimes they were recurring, but there wasn't actually a process how to handle those}."

Furthermore, the transfer interviews add depth by illustrating the illusion of effective failure management. For instance, \PilotSubjectFour described structured root cause analysis meetings, complete with detailed "\emph{five whys analysis}" and formal "\emph{action items documented in Confluence}"; yet despite this apparent rigor, they admitted, "\emph{I don't know if anybody ever really follows up and makes sure that the action items get done}". Similarly, \PilotSubjectThree highlighted the discrepancy between perceived good practice and actual outcomes, stating that beyond taking meeting notes, "\emph{the other guys did not [document anything]. They just talked about it and left the meeting}." These examples strongly illustrate the gap between teams’ perceived effectiveness in managing failures through formal procedures and the ongoing practical reality of unresolved, recurring failures.



\subsection{Theme 5: Challenges within the learning from failures process}

Lack of time and resources.
%%
Subjects share that time and resources are the biggest constraints to learning from failures. 
\SubjectTwo says, "the time is a big issue. When you are involved in a project, you are actually almost hundred percent your time is dedicated for that project and setting and reading or creating new incidents maybe I am pretty sure will take a long time."
\SubjectFive says, "I feel like it's not really feasible for the way we work because most employees are more or less drowned in project work...they don't have enough time" However they add, "But maybe that's even more of a reason to take the time to do that. So it sounds interesting and I would like to try."
\SubjectSix says, "this requires time and they require to take the team out of their normal work and have them in a meeting. And sometimes you can not allow that, but I will actually be in favor of having some kind of time allocated to that. I will actually would be an idea for me to propose to have these kind of discussions. It doesn't need to be maybe, I dunno, once a month to, as an example, during two hours or so. But yeah, I think at the end it comes at the cost of time and personal resources at the end I think that everybody benefit from it. So actually the loss not a loss, but a gain."
\SubjectSeven says,"But what I see it's most of the time, okay, we didn't have time, we need to set up the next project. Always this issue. And I think there's also all this funding, you have only project funding and normally you doing this lessons learned afterward."
\SubjectNine says, "I think if it's regularly and for many people, then I think it would be just another meeting. But if you do it like tailored to milestones for your next project step and you as the project team go into issues, especially for this part, then it might be a huge benefit. If you invite every two weeks to hold DLR for a discussion, then it might not be meaningful."
\SubjectOne says, "we inherited a lot of technical depth here and that is probably the main problem in all this, since there's always, I mean the deadline shifted a lot, but there was always a deadline we need to be finished"
\SubjectOne adds, "all of our problems come from the fact that we don't have so much time. We are not solely software developers, we're also researchers, sometimes project managers, systems engineers. So we do have several roles, each one of us, and I don't know if we would have the time designated to such a process. I mean that's a bad excuse not having the time when we save time by this. Yeah, that's a bad calculation, but at the very beginning it would probably cause some disturbances in our work time schedule."
\SubjectThree says, "Question is given sometimes let's say budget and tip constraints, if that's the deadline, if that's the time, if you can spend the time,...If you sit down with six people for an hour is basically one full day of work is gone. And if you have too many meetings, also the motivation to attend the meetings and make them productive decreases at a certain point." 
\SubjectThree also adds that "the technical debt" is also a constraint.
\SubjectThree adds, "I wouldn't know how to say do this without annoying other people. So the thing is if you just say, okay, now we meet every week, you make another meeting for one hour and then we talk about our reflection, then everyone will just hate you. And then the question is, it's probably not the productive thing to make people hate you and sit in an hour with you."
\SubjectThree adds, "there's also the question where to take the time...I at least would be open to test it to see and then take out if it's something which we can deem valuable."
\SubjectEight says, "I really like discussing ideas and better way to implement them and also learning new things just from informal talks, than preparing a meeting and also have other time slot during your week that interrupts your work. Yeah, I mean it sounds good, but also it has to be practical, It's not something that you have to do something like, I don't know, maybe twice a month or even once a month for me will become a little bit tedious."
\SubjectTen: "I think that's always the problem that you don't have the time to fill these [failure knowledge] out...I think that's probably the problem that you don't have time. That's the same as writing down, taking notes. It's one of the things that takes time and you usually don't have that...I think the entire team has to see these postmortems as sensible and worth the time putting into"
\SubjectFour says, "Of course the main issue is time because I think everywhere you cannot stop much or spend much time thinking about the exciting this issue is and what exciting things I did to solve it and everything. It's part of your job as a software developer. So yeah, time is the main issue there. Got it."
%%



SDLC is different/informal due to research org
\SubjectThree:
"Yeah, definitely. Because your job is usually not the development, it's more like everything other than the development. And so you have the project meeting, you have your paper stuff, you usually have more than one project, you have all the bureaucracy, maybe you have some other additional tasks and so on. So every additional meeting basically puts a big hole in your calendar again."

\SubjectSix:
"In this mission, we don't really have formal requirements so to say. And it was more on kind of a continuation. It was never a full start or launch. So no, we didn't derive new requirements. But again, this [project] is very, we don't follow an [a specific] process where or a V model where we different requirements and so on. Yeah, it was quite informal...I would say that the issues we created could be considered as requirement in this case."

\SubjectSix:
"No, I don't think we have a very formal standard process, at least in our group. Yeah, I mean we are mostly a research institute and we are not a software house, but we don't have very standardized processes or ways to do these things."

\SubjectOne:
"probably big [tech] companies...and all that there in general with a more agile mind than us because here you have those old processes because space is not agile and it's also not wise to do it. Agile, there is a good reason for not doing it agile."

\SubjectEight: 
"we have to do software development and also scientific work. And I'm thinking now that maybe some things that works for [big tech], software factories it doesn't work for us 100\%. So I think some of them probably works, but not sure if they follow the same approaches done by a software factory."

When asked the standardization about the software processes discussed across the agency, \SubjectThree says, 
"I think generally not very many because I know [the agency] is kind of also quite federalized, so all the institutes are their own small kingdoms and collaborate. But the policy can be very institute specific...And we as an institute for software technology, of course, are much more, let's say software people with much more software affinity than maybe some which actually develop more structural stuff. So our processes regarding software are usually more involved than the ones for people where their software is just a tool and not just the purpose of their actual existence."

When asked if they reflect on their failures, \SubjectFour says, "We are not doing that I think...because we are not following this totally agile approach when you are doing, how do they call it? Milestone and yeah, that process, no, we don't do that. Got it. We use some aspect of agile programming, but I think that usually in this kind of space project you don't see total agile. It's not the case."

However, \SubjectFour points out that their research process helps them reflect, "we do both things here. Not only project development but also research. So when you are actually writing for your research, you usually discover some pitfalls or issues or some points that during the test didn't arise, right? It's like because when you are doing a publication, you need good test result, very good documented with the proper methodology and everything. So When you are doing that process, you notice some pit fails and I think that that combining development with research is important to improve your product quality because when you are doing research you cannot lie, you cannot say no, it has a, B, c features, you have to prove that those features are actually there and the numbers don't lie. So yeah, I think that's an interesting opportunity to think about what you are doing and to improve the things you are doing."



Loss of knowledge due to dynamic team changes and inadequate documentation practices
%%
\SubjectTwo talks the challenges of maintainig failure knowledge and lessons learned as members exit team and new members join dynamically:
"That's a complex one. How you will train a team that's changing every six months is this way. Right? I mean the teams here is dynamic and somehow actually literally every six months someone will join and someone will leave not only the intern and the students actually the main workers or to toppers here. Actually which means you repeat it every six months, it's not Yeah, how handle that with the dynamic team."
And \SubjectTwo emphasizes that such failure knowledge and lessons learned , "should be explicitly documented somewhere because sometimes some some experience is just really relate to one person. Sometimes it's the case eventually losing this person is losing the knowledge, losing the lesson learned with him or with her because she worked on many projects, she was the professional one on one topic and then she decided to leave, and some lesson learned, not completely documented, there will be a loss."
\SubjectTwo:
"That's actually knowledge could be such simply lost and the colleague, the employee will leave us after a year or a few months. They might be reachable a few months, but actually after a while they just will not even answer your emails."
\SubjectFive:
"people are leaving quite frequently and their knowledge is kind of lost. I think it would really make sense, but I don't see it that structured in our current processes. So something like lessons learned would definitely be helpful."
\SubjectNine:
"people are only there for a limited time, so knowledge gets lost and that's something really bad...there's so much knowledge was just gone within seconds"
\SubjectTwo:
"knowledge could be lost because they are not well documented...and then actually it's gone because there's no process to say no, part of your project is to write lesson learned...that's the most problematic"
\SubjectSeven says:
"I have the feeling that we loses right now since the wiki was new there was very good contributions but right now I think it's not available anymore. I think there's the spirit of the wiki to contribute. It's different when you have a wiki with a lot of pages where you didn't find anything anymore. Because the search Is bad. Wiki, which is fresh and you are the first one to share information."
\SubjectNine says:
"There still should be some kind of written solutions. So even with discussions and...other stuff which might be helpful for current situations, but it still should be somewhere document, so someone has to write at least something. Yeah, that's one issue. I just think that even without all this practices, that still not everything is captured somewhere."






Challenge of distributed knowledge
%%
\SubjectFive:
But to be honest, I don't have an idea how you could do this because we have a lot of knowledge somewhere in different places in GitLab, in the wiki, in the team sites, in the intranet, I don't know. And people don't know that it, it's there and they don't look at it. So it doesn't really help in the end. And I think that's always a problem with that kind of knowledge. It doesn't help if nobody knows that it's there."



\SubjectEight: "if you have to coordinate people from that is working from different projects, I think that could be a problem. But if it is like a project level, maybe it's easier."


\SubjectSeven: "Political issues that your institutes, you have your institutes heads and you have always this border between these institutes and by political issues. Normally when you are on the low level and designing your process, then you can share this experiences. But on the high levels always this okay, why we should share our knowledge with other institute."



SUbject 7:
"
I have the feeling that we loses right now since the wiki was new there was very good contributions but right now I think it's not available anymore. I think there's the spirit of the wiki to contribute. It's different when you have a wiki with a lot of pages where you didn't find anything anymore. Because the search Is bad. Wiki, which is fresh and you are the first one to share information.
"

Subject 5:
"
I really had the issue in the beginning that I didn't know where to find stuff I didn't really know about. I knew that there is a GitLab, but I didn't know what was documented in GitLab, what was documented in the wiki and what was documented on the team side and what was discussed in which meeting. But that's also really project dependent, but I think something like how are the processes and how do you do it in this project would be really helpful if you start.
"

Subject 1:
"Subject 1, one of the senior engineers, contradicts the rest of the knowledge transfer practices shared by saying, "Only if the person who either fixed it or who was there in the discussion with members only then this could happen. I never experienced that, to be honest, that someone says like, oh yeah, we had this issue before and we fixed it like this and this and we can do it, but there's not a process to look it up to say, okay, let's just ask a database might be that this was already fixed." But they recount a time where they were able to help with an issue based on past experience, "It was more like someone called me and asked, here I have this and that issue. Have you ever experienced that? And I basically helped them, but further than that, we didn't take any measures to prevent that" - Showing that this may not really be a general practice.
"

Subject 1:
"there are some software engineering guidelines from the [agency] and I think they state that in some form issues need to be documented...And software development in the [agency] should follow, follow this software engineering guidelines, but they are not enforced to do and that's probably the problem. So since the beginning, since I'm here and working on the software project, we were trying to implement the software engineering guidelines, but what we actually did is we said, we went through the guidelines and said, okay, this is fulfilled by this. And I think for this specific part we said, okay, we can handle that with our GitLab issues. But actually I think the software engineering guidelines are technology agnostic and that point and just says you have to have a process."

\SubjectTwo
explained that despite this tool being available, recurring failures persist because knowledge sharing is limited, especially among newer engineers:
\myinlinequote{I see that happened again and again because most of the young engineers, software engineers coming directly from the university, they didn't have the experience and the sharing of experiences is limited.}

\myparagraph{Transferability}
The pilot study supports the case study findings by emphasizing that lack of time and resources are significant constraints preventing effective learning from failures. Both studies highlight that daily workload pressures severely limit the time teams can allocate to structured reflection or systematic learning activities. For instance, \PilotSubjectOne notes, "\emph{usually someone will write [documentation]...but especially on our team right now, we don't have time to write new people documentation}," aligning closely with the case study participants (\SubjectOne, \SubjectTwo, \SubjectSix), who similarly cited time and resource constraints as major barriers. Both studies also reveal that although formal methods, like structured root-cause analyses or reflective practices, might exist in theory or as good practices, in reality these activities are frequently sidelined due to immediate demands of ongoing development and workload pressures.

The pilot study also provides insights into organizational pressures that compound these challenges, highlighting urgency-driven environments and cultural differences across organizations. For instance, participants described how issues requiring immediate attention prevent structured reflection: "\emph{We don't necessarily have separate sessions to teach [about failures]...we have to start working immediately}" (\PilotTeam), and "\emph{We're usually writing code, integrating, making sure things are working, and that eats up all our time}" (\PilotSubjectOne). Participants also introduced the notion that organizational structure affects the feasibility of structured learning—software-focused organizations reportedly had "\emph{much more civilized software engineering practices}" (\PilotSubjectThree), suggesting organizational culture and product focus significantly influence the practicality and success of structured failure management processes. These findings add valuable depth to the case study by highlighting that organizational context and culture strongly impact the effectiveness of learning from failures.

\subsection{Theme 6: Perceived benefits of learning from failures} 
All subjects of the case study share that it would be beneficial to have a process to learn from failures. 

Most subjects (8/10) mention that it would be beneficial to discuss failures and to gather lessons learned.

Most subjects (8/10) mention that it would be beneficial to document lessons learned.

Most subjects (8/10) mention that it would be beneficial to share lessons learned.

Almost all subjects (9/10) mention that it would be beneficial to reference lessons learned.



\subsection{Theme 7: Role of automation to aid learning from failures}

\JD{Move all of Theme 7 this to an appendix}
\DA{
Relevant lit:
1)
Knowledge management in software engineering: A systematic review of studied concepts, findings and research methods used - "...39 reports of lessons learned. More than half of the empirical studies were case studies."


2) Tool support for disseminating and improving development practices. 
Also there's another paper that we reference in FAIL about tech challenges to learning from failures - aka database etc, that we use to claim that back in the days relevant tech didn't exist which made it harder.
"
Another problem is that, even if postmortems are performed, information is seldom shared
across project boundaries (Birk et al. 2002; Glass 2002a; von Zedtwitz 2002), with the result
that the only vessel for knowledge transfer is the individual practitioner moving between
projects. Methods for analyzing postmortem data for use on an organizational level exist, but
carry high costs (Dingsøyr et al. 2007; Schalken et al. 2006). The project managers, who are
the driving force behind selecting the practices to be used in a specific project, might or might
not be involved in the learning experience of another project. This problem is compounded
by the fact that few organizations have procedures or structures in place to enable sharing of
information (Glass 2001; Verner and Evanco 2005; von Zedtwitz 2002). This can be devastating, as good practices are highly dependent on project characteristics, i.e., what works
for one project might not be suitable for another (Davis and Zowghi 2004; Glass 2002b).
Relying only on word-of-mouth rumors, good practices conveyed out of context with little or
no additional information can create more problems than they solve.
"

3) 
A method to draw lessons from project postmortem databases
A framework for filling postmortem reports. Authors claim if this is followed, then a large set of them could provide quantitative lessons for improvement.
}


